Approximate Stream Analytics in Apache Flink and Apache Spark Streaming

Approximate computing aims for efficient execution of workflows where an approximate output is sufficient instead of the exact output. The idea behind approximate computing is to compute over a representative sample instead of the entire input dataset. Thus, approximate computing - based on the chosen sample size - can make a systematic trade-off between the output accuracy and computation efficiency. Unfortunately, the state-of-the-art systems for approximate computing primarily target batch analytics, where the input data remains unchanged during the course of sampling. Thus, they are not well-suited for stream analytics. This motivated the design of StreamApprox - a stream analytics system for approximate computing. To realize this idea, we designed an online stratified reservoir sampling algorithm to produce approximate output with rigorous error bounds. Importantly, our proposed algorithm is generic and can be applied to two prominent types of stream processing systems: (1) batched stream processing such as Apache Spark Streaming, and (2) pipelined stream processing such as Apache Flink. We evaluated StreamApprox using a set of microbenchmarks and real-world case studies. Our results show that Spark- and Flink-based StreamApprox systems achieve a speedup of $1.15\times$-$3\times$ compared to the respective native Spark Streaming and Flink executions, with varying sampling fraction of $80\%$ to $10\%$. Furthermore, we have also implemented an improved baseline in addition to the native execution baseline - a Spark-based approximate computing system leveraging the existing sampling modules in Apache Spark. Compared to the improved baseline, our results show that StreamApprox achieves a speedup $1.1\times$-$2.4\times$ while maintaining the same accuracy level.

==> background.tex <==
\section{Background}
\label{sec:background}



\myparagraph{Incremental Computation}

\myparagraph{Approximate Computation}



==> errorCalculation.tex <==
\section{Approximation and Error Bound}

\subsection{Error calculation for Aggregate functions}
In a streaming environment where the data comes in from different strata, the calculations mostly involve a statistics within a particular strata i.e, instead of an aggregation function over the whole population, we are mostly interested in an aggregation within a strata. For example, if the population is divided into strata based on country, then how many times a word 'health' comes in each strata (each country) would let us know how frequently health-concerned topics are discussed in each country.

\subsubsection{Multi Stage Stratified Sampling}
Stratified Sampling is a special case of two stage sampling. A stratified random sample is a census of the primary units (stratas) followed by a simple random sampling of the secondary units within each primary unit [cite]. The division of population to stratas form the first stage. Each strata might contain many items out of which few items are sampled. This forms the second stage of a general stratified sampling.\\

\begin{figure}[t]
\centering
\includegraphics[scale=0.60]{figuresTex/figures/StrataBlocks}
\caption{Each strata consists of blocks of data and each block contains many pages. Each sampled block is processed by a Map Task.}
\label{fig:StrataBlocks}
\end{figure}

Our computations are strata-specific i.e, we are interested to know only the statistics within a strata. In our approach, the data in each strata is partitioned into several input data blocks. The first stage of sampling is to sample input blocks in the strata. In figure \ref{fig:StrataBlocks} Strata S1 has blocks b1,b2,b3 and b4. Each blocks contain many pages. The blocks b1 and b3 are sampled. Let the total Strata size be S and it is partitioned into B blocks. Suppose each block i consists of $P_{i}$ units (eg: Web pages) so that  $S = \sum_{i=1}^B P_{i} $. Further, let each unit j in block i has an associated value $v_{ij}$ and we want to count the sum of these values accross the strata i.e, $\sum_{i=1}^B \sum_{j=1}^{P_{i}} v_{ij}$.

For a word count example to find number of words in a web page specific to a strata (for example all .com web pages is a strata, all .de is another etc), we must find count of words in each of the pages of sampled blocks within the strata.
Basically in sampling, the sample "represents" the total population. That means each sampling unit (block) "represents" certain number of units in the total population. Suppose out of 300 blocks, we sample 30 blocks. It means each of the block is equivalent to 10 blocks in the total population or each block has a the sampling weight of 10. The sampling weight for an observation unit is always the reciprocal of the probability that the observation unit is included in the sample (in without-replacement sampling) i.e reciprocal of 30/300 is the weight here. \\

Multi-stage sampling works as follows: Suppose the whole population(window) has $S_{x}$ strata and each strata has $B_{x}$ blocks. 
A word count program would want to find the count within each strata i.e, a total count of whole population might not be needed since computations are within each strata. So consider one Strata S divided into 'B' blocks. From these B blocks, 'b' blocks are sampled. Here b blocks have a weightage $\frac{B}{b}$. Thus word count within a strata could be expressed as
$\frac{B}{b} \sum_{i=1}^b  W_{i} $ where $W_{i}$ is the word count in $i^{th}$ block.
Suppose $i^{th}$ block has $P_{i}$ pages. So above equation could be expressed as 
$\frac{B}{b} \sum_{i=1}^b  (\sum_{j=1}^{P_{i}}  w_{ij}) $ where $w_{ij}$ is word count in $j^{th}$ page of $i^{th}$ block.
But it is not the real word count obtained by processing pages in all blocks, and is an \textit{estimated} word count using sample of blocks and weightage of sample. So there could be a possible error due to sampling. Thus the total word count within a strata could be expressed by including a margin of error as:\\

\begin{equation}\label{eq:sum}
\frac{B}{b} \sum\limits_{i=1}^b (\sum\limits_{j=1}^{P_{i}} w_{ij}) \pm \epsilon 
\end{equation}

The error bound $\epsilon$ can be defined as:
\begin{equation}\label{eq:epsilon}
\epsilon_{t_{n-1},1-\tfrac{\alpha}{2} } \sqrt{\widehat{Var(\tau)}}
\end{equation}
where $\widehat{Var(\tau)}$ is the estimated variance for sum. The Standard error in Stratified Sampling is calculated based on the variance. For example, the standard error in population sum is the square root of variance in the population sum. \\

Based on statistical theories for stratified sampling, when a population has 'H' stratas and $N_{h}$ be the units in $h^{th}$ strata, and $n_{h}$ 
be the number of units sampled from $h^{th}$, then the estimated variance of sum for the \textit{whole population} \cite{samplingBySteve} is represented as:

\begin{equation}\label{eq:variance_population}
\widehat{Var(\tau)} = \sum\limits_{i=1}^H (1 - \dfrac{n_{h}}{N_{h}}) N_{h}^2 *  \dfrac{s^2_{h}}{n_{h}}
\end{equation}
where $s^2_{h}$ is the population variance in stratum h.\\

Since our computations are specific to a strata, we need to find the estimated variance within each strata. Suppose the strata has B blocks, and b blocks are sampled, the above equation could be re-phrased and simplified to find the estimated variance of sum \textit{within a strata }as:
\begin{equation}\label{eq:variance_strataSpecific}
\widehat{Var(\tau)} =  B(B - b) *  \dfrac{s^2}{b}
\end{equation}
where $s^2$ is the population variance within the stratum.\\

\subsubsection{Applying Sampling in Map-Reduce}
Streaming data could be processed in batches of sliding windows. Each batch could be considered as a window which is divided into stratas. While applying strata specific aggregate functions to this batch of data, approximation could be done for the result within each strata. For computation of aggregate functions like sum, average etc within the the strata, we could make use of a Map-Reduce framework. The components of stratified sampling could be mapped to components in a Map-Reduce framework. \\

Consider the example mentioned before in a word count problem to find how frequently health related topics are discussed in each country. For this, the batch of data(or window) has to be stratified based on country specific url e.g, .de for Germany, .uk for UK etc. Since the web-pages in each country would be so large in number, the strata would be divided into blocks of web-pages. Each block consists of many web-pages. We do sampling of the blocks to select few blocks from each strata. This block-sampling is done proportional to the size of strata. The sampled blocks consists of web-pages and all web-pages are processed to count the number of times word 'health' appears in them. As a next stage of sampling, we could chose a sub-set of webpages in each sampled block, but we choose to process all of them for better accuracy.\\

The Map phase of an MR framework could count the occurance of the word in each page, and Reduce phase could sum the count. For approximate computing, the Map phase produces an output <word, v> for the pages in the sampled blocks, where v is an associated value. The reduce phase produces an approximate sum of how many times word occurs in the whole strata, based on a relative computation from the sampled blocks. The reduce phase also incorporates the error bound as given in the equation \ref{eq:sum}.
In an MR job which produces x intermediate keys, there needs to be x distinct computations for finding the approximate sum of each of these keys. Here the Map phase would produce z different <key,value> pairs and the reduce phase would produce x approximate sums, each with its own error bound as: $<k1,v1> \pm \epsilon_{1},  <k_{2},v_{2}> \pm \epsilon_{2}   ...   <k_{x},v_{x}> \pm \epsilon_{x}$.\\

The MR framework processes only fewer amount of data, i.e it processes only the samples in each strata, instead of processing the whole strata. Thus computation cost is greatly reduced. Further, the confidence interval of the computation could be calculated using the algorithm for Error bound discussed in next section.

\subsection{Algorithm to find Error Bound}
The uncertainity of the sampling method is described by the confidence level(CI). Using the same sampling method, if we take multiple samples, the proportion that the parameter considered falls in the interval mentioned will be the level of confidence. For example 95 \% CI means that we are 95 \% confident that the true value of parameter falls in the interval.

\begin{equation}\label{eq:confInterval}
CI = Sample Statistic \pm MarginOfError\\
\end{equation}
where CI is the Confidence Interval
Sample statistic is any statistic of the sample we consider, for example, sample sum or sample mean.
\begin{equation}\label{eq:marginErr}
MarginOfError = CriticalValue * StandardError
\end{equation}
where the Standard error is calculated based on teh sample statistic

Critical value is a factor used to compute the margin of error. It can be expressed as t-score when the sampling distribution is normal. Critical value is same as the t-score with 2 conditions:

\textit{1. Degree of freedom = sample size -1}

\textit{2. Cumulative probability = critical probabilty}\\

When degrees of freedom increase, the t-distribution tends to move closer to the standard normal distribution and t-distribution with infinite degrees of freedom is same as the standard normal distribution.
\begin{equation}\label{eq:CrProb}
Critical Probability = 1-\alpha/2
\end{equation}
where $\alpha$ = 1- confidence interval/100. Using a t Distribution Calculator, we can calculate the critical value for a given t-score with degree of freedom and cumulative value. For example, for 95\% confidence Interval for sample size 900, the cumulative probability is 0.975 and critical value is 1.96. 



==> figuresTex/fig-accuracy-benchmark.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.35\textwidth]{figuresTex/figures/accuracy-comparison-benchmark.eps}
\caption{The accuracy loss of projecttitle,  Spark based simple random sampling,  and Spark based stratified sampling.}
\label{fig:accuracy-benchmark}
\end{figure}


==> figuresTex/fig-accuracy-benchmarks.tex <==
\begin{figure}
\centering
\includegraphics [width=0.35\textwidth]{figuresTex/figures/accuracy-benchmarks.eps}
\caption{The accuracy loss comparison between sampling systems with varying sampling fractions. The sliding window size is 10 seconds, and each sliding step is 5 seconds.}
%\vspace{-5mm}
\label{fig:accuracy-benchmarks}
\end{figure}


==> figuresTex/fig-accuracy-windowsizes.tex <==
\begin{figure}
\centering
\includegraphics [width=0.35\textwidth]{figuresTex/figures/accuracy-windowsizes.eps}
\caption{The accuracy loss comparison between sampling systems with varying window sizes. The sampling fraction is set to 60\%.}
%\vspace{-5mm}
\label{fig:accuracy-windowsizes}
\end{figure}


==> figuresTex/fig-arrival-rates.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{figuresTex/figures/memoization.eps}
\caption{Effect of changing arrival rate on memoization }
\label{fig:arrival-rate}
\end{figure}


==> figuresTex/fig-arriving-rate-fluctuation.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{figuresTex/figures/arriving-rate-fluctuation.eps}
\caption{The mean of the input data stream with fluctuating arrival rates. Window interval $w = 10\ seconds$ and slide interval $\delta = 5\ seconds$.}
\label{fig:arriving-rate-fluctuation}
\end{figure}

==> figuresTex/fig-case-studies.tex <==
\begin{figure*}[t]
\centering
\includegraphics [width=1\textwidth]{figuresTex/figures/case-studies.eps}
\caption{{\em (a)} Peak throughput comparison between Inc, Approx, \projecttitle, and native Spark Streaming with the sampling fraction is set to 60\%. {\em (b) \& (c)} The effect of varying sampling fractions on throughput and accuracy with end-to-end latency $350ms$}
\vspace{-5mm}
\label{fig:case-studies}
\end{figure*}


==> figuresTex/fig-computation-model.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.35]{figuresTex/figures/computation-model}
\caption{Sliding window computation over data stream}
\label{fig:computation-model}
\end{figure}

==> figuresTex/fig-error.tex <==
\begin{figure}[htp]
\centering
\includegraphics[width=0.45\textwidth]{plots/accuracy-incapprox.eps}
\caption{Accuracy loss in processing the NetFlow and Tweet stream data under different sampling rates. Sampling rates directly correspond to sample sizes, e.g., a rate of 5\% corresponds to the sample size of 5\%.
}
\label{fig:error}
\end{figure}


==> figuresTex/fig-eval-slide-interval.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.5]{figuresTex/figures/slide-interval}
\caption{Effect of slide interval on memoization}
\label{fig:slideInterval}
\end{figure}


==> figuresTex/fig-evaluation.tex <==
\begin{figure*}[t]
\centering
\includegraphics [width=1\textwidth]{figuresTex/figures/mem-evaluation.eps}
\caption{Effect of various parameters such as sample size, slide interval, window size and arrival rate on memoization}
\vspace{-5mm}
\label{fig:evaluation}
\end{figure*}


==> figuresTex/fig-implementation-flink.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{figuresTex/figures/implementation-flink.png}
\caption{Architecture of Flink-based \projecttitle prototype (shaded boxes depict the implemented modules).}
\label{fig:flink-streamapprox-implementation}
\end{figure}

==> figuresTex/fig-micro-benchmarks.tex <==
\begin{figure*}[t]
\centering
\includegraphics [width=1\textwidth]{figuresTex/figures/micro-benchmarks.eps}
\caption{The mean values of the received data items produced by different sampling systems every 5 seconds during a 10-minute observation. The sliding window size is 10 seconds, and each sliding step is 5 seconds.}
\vspace{-5mm}
\label{fig:micro-benchmarks}
\end{figure*}


==> figuresTex/fig-poisson-accuracy-benchmarks.tex <==
\begin{figure}
	\centering
	\includegraphics [width=0.35\textwidth]{figuresTex/figures/poisson-accuracy-comparison.eps}
	\caption{The accuracy loss comparison between sampling systems with the Poisson distribution dataset.}
	%\vspace{-5mm}
	\label{fig:poisson-accuracy-benchmarks}
\end{figure}



==> figuresTex/fig-sac-slide.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.33]{figuresTex/figures/sliding-sac}
\caption{Run data-parallel job incrementally}
\label{fig:data-parallel-sac}
\end{figure}


==> figuresTex/fig-sample-size.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.6]{figuresTex/figures/Sample-size}
\caption{Effect of sample size and arrival rate on memoization}
\label{fig:sample-size}
\end{figure}



==> figuresTex/fig-sampling-model.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.22]{figuresTex/figures/sampling-model.png}
\caption{Model of a sampling-batched stream processing system}
\label{fig:sampling-model}
\end{figure}

==> figuresTex/fig-scalability-benchmarks.tex <==
\begin{figure}
\centering
\includegraphics [width=0.35\textwidth]{figuresTex/figures/scalability-benchmarks.eps}
\caption{The throughput comparison between sampling systems with varying number of CPU cores and nodes. The sliding window size is 10 seconds, and each sliding step is 5 seconds.}
%\vspace{-5mm}
\label{fig:scalability-benchmarks}
\end{figure}


==> figuresTex/fig-simplified-sampling.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.36]{figuresTex/figures/simplified-sampling.png}
\caption{Simplified sampling approach with a Pub/Sub aggregator.}
\label{fig:simplified-sampling}
\end{figure}

==> figuresTex/fig-strata-blocks.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.60]{figuresTex/figures/StrataBlocks}
\caption{Each strata consists of blocks of data items. Each sampled block is processed by a Map Task.}
\label{fig:StrataBlocks}
\end{figure}

==> figuresTex/fig-throughput-accuracy-benchmarks.tex <==
\begin{figure}
\centering
\includegraphics [width=0.35\textwidth]{figuresTex/figures/throughput-accuracy-benchmarks.eps}
\caption{The throughput comparison between sampling systems. The sliding window size is 10 seconds, and each sliding step is 5 seconds.}
%\vspace{-5mm}
\label{fig:throughput-accuracy-benchmarks}
\end{figure}


==> figuresTex/fig-throughput-batch-interval-benchmarks.tex <==
\begin{figure}
\centering
\includegraphics [width=0.35\textwidth]{figuresTex/figures/throughput-batch-interval-benchmarks.eps}
\caption{The throughput comparison between sampling systems with varying batch intervals. The sliding window size is 10 seconds, and each sliding step is 5 seconds.}
%\vspace{-5mm}
\label{fig:throughput-batch-interval-benchmarks}
\end{figure}


==> figuresTex/fig-throughput-benchmark.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{figuresTex/figures/throughput-benchmark.eps}
\caption{Peak throughput comparison between \projecttitle,  Spark based simple random sampling, and Spark based stratified sampling.}
\label{fig:throughput-benchmark}
\end{figure}


==> figuresTex/fig-throughput-sampling-fraction-benchmarks.tex <==
\begin{figure}
\centering
\includegraphics [width=0.35\textwidth]{figuresTex/figures/throughput-sampling-fraction-benchmarks.eps}
\caption{The throughput comparison between sampling systems with varying sampling fractions. The sliding window size is 10 seconds, and each sliding step is 5 seconds.}
%\vspace{-5mm}
\label{fig:throughput-sampling-fraction-benchmarks}
\end{figure}


==> figuresTex/fig-throughput-windowsizes.tex <==
\begin{figure}
\centering
\includegraphics [width=0.35\textwidth]{figuresTex/figures/throughput-windowsizes.eps}
\caption{The throughput  comparison between sampling systems with varying window sizes. The sampling fraction is set to 60\%.}
%\vspace{-5mm}
\label{fig:throughput-windowsizes}
\end{figure}


==> figuresTex/fig-throughput.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{plots/throughput-incapprox.eps}
\caption{Throughput comparison between Inc, Approx, \projecttitle and native Spark Streaming when processing NetFlow and Tweet stream data.}
\label{fig:throughput}
\end{figure}


==> figuresTex/fig-varying-window-size.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.54]{figuresTex/figures/Varying-window-size}
\caption{Effect of varying window size on memoization}
\label{fig:varying-window-size}
\end{figure}



==> scheduler.tex <==
\section{Thread Scheduler}
\label{sec:scheduler}
